Adversarial Counterfactual Visual Explanations

Counterfactual explanations and adversarial attacks have a related goal: flipping output labels with minimal perturbations regardless of their characteristics. Yet, adversarial attacks cannot be used directly in a counterfactual explanation perspective, as such perturbations are perceived as noise and not as actionable and understandable image modifications. Building on the robust learning literature, this paper proposes an elegant method to turn adversarial attacks into semantically meaningful perturbations, without modifying the classifiers to explain. The proposed approach hypothesizes that Denoising Diffusion Probabilistic Models are excellent regularizers for avoiding high-frequency and out-of-distribution perturbations when generating adversarial attacks. The paper's key idea is to build attacks through a diffusion model to polish them. This allows studying the target model regardless of its robustification level. Extensive experimentation shows the advantages of our counterfactual explanation approach over current State-of-the-Art in multiple testbeds.

==> sections/tables-rebuttal/filtering.tex <==
% \begin{table}[t]
%     \centering
%     \footnotesize
%     \scalebox{0.8}{
%     \begin{tabular}{c|cccc} \toprule
%         $\tau \backslash ^\text{RT}$    &   25 &   50 &  100 &  200 \\ \midrule
%         5   & \textbf{85.5 (80.9)} & 90.4 (72.9) & 93.6 (24.2) & 95.7 (0.0) \\
%         10  & 68.5 (67.5) & \textbf{85.5 (81.9)} & 91.9 (76.9) & 94.9 (36.9) \\
%         20  & 2.0 (2.2)  & 68.0 (67.4) & \textbf{85.1 (82.0)} & 91.7 (77.6) \\ \bottomrule
%     \end{tabular}}
%     \vspace{-0.1cm}
%     \caption{\textbf{Filtering recovery ratio.} \emph{Initial Timesteps} ($\tau$). \emph{Rescaled Timesteps} (RT). The number in parentheses are fraction of recovered samples with adversarial noise (bound \nicefrac{32}{255}) on ImageNet.
%     }
%     \label{tab:t1}
% \end{table}

% \begin{table}[t]
%     \centering
%     \footnotesize
%     \scalebox{0.8}{
%     \begin{tabular}{c|cccc} \toprule
%         Threshold & sFID & FS    & COUT & CD  \\ \midrule
%         None      & 9.09 & 0.765 &0.532 & \textbf{2.66} \\
%         0.05      & 6.83 & 0.787 &0.547 & 3.12 \\
%         0.10      & 5.23 & 0.792 &0.565 & 2.75 \\
%         0.15      & \textbf{4.62} & \textbf{0.797} &\textbf{0.564} & 2.82 \\ \midrule
%         DiME      & 5.89 & 0.671 &0.444 & 3.27 \\ \bottomrule
%     \end{tabular}}
%     \vspace{-0.1cm}
%     \caption{Threshold ablation on CelebA (Age) with $l_2$ distance loss.}
%     \label{tab:t2}
% \end{table}

\begin{table}[t]
    \centering
    \footnotesize
    \scalebox{0.8}{
    \begin{tabular}{c|cccc|c} \toprule
        Threshoold & None & 0.05 & 0.10 & 0.15 & DiME \\ \midrule
        sFID       & 9.09 & 6.83 & 5.23 & \textbf{4.62} & 5.89 \\
        FS         &0.765 & 0.787& 0.792& \textbf{0.797}& 0.671\\
        COUT       & 0.532& 0.547& 0.565& \textbf{0.564}& 0.444\\
        CD         &\textbf{2.66}& 3.12& 2.75& 2.82& 3.27 \\ \bottomrule
    \end{tabular}}
    \vspace{-0.1cm}
    \caption{Threshold ablation on CelebA (Age) with $l_2$ distance loss.}
    \label{tab:t2}
\end{table}


\begin{table}[t]
    \centering
    \footnotesize
    \scalebox{0.8}{
    \begin{tabular}{c|cccc} \toprule
        Method      & sFID             & FVA               & FS                & MNAC \\ \midrule
        DiME        & 4.89 $\pm$ 0.08 & 0.982 $\pm$ 0.132 & 0.705 $\pm$ 0.086 & 3.68 $\pm$ 1.86 \\
        ACE + $l_1$ & 3.97 $\pm$ 0.11 & 0.999 $\pm$ 0.019 & 0.874 $\pm$ 0.069 & 2.93 $\pm$ 1.66 \\
        ACE + $l_2$ & 4.56 $\pm$ 0.11 & 0.999 $\pm$ 0.014 & 0.867 $\pm$ 0.066 & 2.77 $\pm$ 1.58 \\ \bottomrule
    \end{tabular}}
    \vspace{-0.1cm}
    \caption{Mean $\pm$ Standard Deviation on CelebA (Smile).}
    \label{tab:t3}
     \vspace{-0.3cm}
\end{table}

==> sections/tables/ablating-simsiam-metric.tex <==
\begin{table}[t]
    \centering
    \footnotesize
    \begin{tabular}{c|ccccc} \toprule
        %\multicolumn{6}{c}{\textbf{Celeb A}} \\\midrule
        Method        & FID  & sFID & FVA  & MNAC & FR \\ \midrule
        GD            & \\
        C\&W          & \\
        PGD   (ours)  & \\ \bottomrule
    \end{tabular}
    \caption{\textbf{Ablation study 3.} Here we show the effect of the adversarial attack.}
    \label{tab:ablation-simsiam}
\end{table}

==> sections/tables/ablation-adv.tex <==
\begin{table}[b]
    \centering
    \footnotesize
    \begin{tabular}{c|ccccc} \toprule
        %\multicolumn{6}{c}{\textbf{Celeb A}} \\\midrule
        Method        & FID  & sFID & FVA  & MNAC & FR \\ \midrule
        GD            & \\
        C\&W          & \\
        PGD           & \\ \bottomrule
    \end{tabular}
    \caption{\textbf{Ablation study 2.} Here we show the effect of the adversarial attack.}
    \label{tab:ablation-adv}
\end{table}

==> sections/tables/filtering.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{c|c|cccc} \toprule
        \multirow{5}{*}{\rotatebox[origin=c]{90}{$\epsilon=\nicefrac{0}{255}$}} & IT & \multicolumn{4}{|c}{Sampling Steps}  \\ \cmidrule{2-6}
        &     &   25 &   50 &  100 &  200 \\ \cmidrule{2-6}
        & 5   & 85.5 & 90.4 & 93.6 & 95.7 \\
        & 10  & 68.5 & 85.5 & 91.9 & 94.9 \\
        & 20  & 2.0  & 68.0 & 85.1 & 91.7 \\ \bottomrule\toprule
        \multirow{5}{*}{\rotatebox[origin=c]{90}{$\epsilon=\nicefrac{8}{255}$}} & IT & \multicolumn{4}{|c}{Sampling Steps}  \\ \cmidrule{2-6}
        &     &   25 &   50 &  100 &  200 \\ \cmidrule{2-6}
        & 5   & 82.4 & 81.9 & 58.5 & 13.2 \\
        & 10  & 67.9 & 83.1 & 84.8 & 66.3 \\
        & 20  & 2.2  & 67.5 & 83.0 & 84.8 \\ \bottomrule\toprule
        \multirow{5}{*}{\rotatebox[origin=c]{90}{$\epsilon=\nicefrac{16}{255}$}} & IT & \multicolumn{4}{|c}{Sampling Steps}  \\ \cmidrule{2-6}
        &     &   25 &   50 &  100 &  200 \\ \cmidrule{2-6}
        & 5   & 80.9 & 75.1 & 29.8 &  0.0 \\
        & 10  & 67.6 & 82.3 & 78.7 & 42.2 \\
        & 20  & 2.1  & 68.0 & 82.2 & 78.4 \\ \bottomrule\toprule
        \multirow{5}{*}{\rotatebox[origin=c]{90}{$\epsilon=\nicefrac{32}{255}$}} & IT & \multicolumn{4}{|c}{Sampling Steps}  \\ \cmidrule{2-6}
        &     &   25 &   50 &  100 &  200 \\ \cmidrule{2-6}
        & 5   & 80.9 & 72.9 & 24.2 &  0.0 \\
        & 10  & 67.5 & 81.9 & 76.9 & 36.9 \\
        & 20  & 2.2  & 67.4 & 82.0 & 77.6 \\ \bottomrule
        
    \end{tabular}
    \caption{\textbf{Filtering recovery.} Images ratio prediction recovery after perturbing it with different \emph{Initial Timesteps} (IT) under different Number of \emph{Sampling Step}. The $\epsilon$ stands for the attack PGD attack strength.}
    \label{tab:my_label}
\end{table}

==> sections/tables/threshold.tex <==
\begin{table}[t]
    \centering
    \footnotesize
    \begin{tabular}{c|cccc} \toprule
        Threshold & sFID & FS    & COUT & CD  \\ \midrule
        None      & 9.09 & 0.765 &0.532 & \textbf{2.66} \\
        0.05      & 6.83 & 0.787 &0.547 & 3.12 \\
        0.10      & 5.23 & 0.792 &0.565 & 2.75 \\
        0.15      & \textbf{4.62} & \textbf{0.797} &\textbf{0.564} & 2.82 \\ \midrule
        DiME      & 5.89 & 0.671 &0.444 & 3.27 \\ \bottomrule
    \end{tabular}
    \vspace{-0.1cm}
    \caption{Threshold ablation on CelebA (Age) with $l_2$ distance loss.}
    \label{tab-sup:t2}
\end{table}
